Towards efficient keyword spotting using spike-based time difference encoders

Keyword spotting in edge devices is becoming increasingly important as voice-activated assistants are widely used. However, its deployment is often limited by the extreme low-power constraints of the target embedded systems. Here, we explore the Temporal Difference Encoder (TDE) performance in keyword spotting. This recent neuron model encodes the time difference in instantaneous frequency and spike count to perform efficient keyword spotting with neuromorphic processors. We use the TIdigits dataset of spoken digits with a formant decomposition and rate-based encoding into spikes. We compare three Spiking Neural Networks (SNNs) architectures to learn and classify spatio-temporal signals. The proposed SNN architectures are made of three layers with variation in its hidden layer composed of either (1) feedforward TDE, (2) feedforward Current-Based Leaky Integrate-and-Fire (CuBa-LIF), or (3) recurrent CuBa-LIF neurons. We first show that the spike trains of the frequency-converted spoken digits have a large amount of information in the temporal domain, reinforcing the importance of better exploiting temporal encoding for such a task. We then train the three SNNs with the same number of synaptic weights to quantify and compare their performance based on the accuracy and synaptic operations. The resulting accuracy of the feedforward TDE network (89%) is higher than the feedforward CuBa-LIF network (71%) and close to the recurrent CuBa-LIF network (91%). However, the feedforward TDE-based network performs 92% fewer synaptic operations than the recurrent CuBa-LIF network with the same amount of synapses. In addition, the results of the TDE network are highly interpretable and correlated with the frequency and timescale features of the spoken keywords in the dataset. Our findings suggest that the TDE is a promising neuron model for scalable event-driven processing of spatio-temporal patterns.

==> tab/tab_comparison2.tex <==

% Energy-computations TABLE
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table}[]
\caption{Comparative table of spikes, synaptic operations per keyword averaged over the whole dataset for the tested architectures after training in the decoding the whole dataset.}
\label{tab:net_allComp}
\begin{tabular}{llllllll}
 &  & \multicolumn{2}{l}{\textbf{TDE}} & \multicolumn{2}{l}{\textbf{LIFrec}} & \multicolumn{2}{l}{\textbf{LIF}} \\ \hline 
\multicolumn{2}{l}{\textbf{Accuracy}} & \multicolumn{2}{c}{87.86 (1.12)} & \multicolumn{2}{c}{90.04 (0.8)} & \multicolumn{2}{c}{71.59 (2.72)}  \\ \hline 
\multicolumn{2}{l}{\textbf{\# cells (L1)}} & \multicolumn{2}{c}{540} & \multicolumn{2}{c}{65} & \multicolumn{2}{c}{163} \\ \hline
\multicolumn{2}{l}{\textbf{Synaptic connections}} & \multicolumn{2}{c}{7020} & \multicolumn{2}{c}{7020} & \multicolumn{2}{c}{7009} \\ \hline
\multicolumn{2}{l}{\textbf{Spikes}} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff } & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff } \\ \hline
\textbf{Layer} & L0 & 77 & 0.00\% & 77 &  & 77 & 0.00\% \\
\textbf{} & L1 & 975 & -55.95\% & 2213 &  & 757 & -65.78\% \\
\textbf{} & L2 & 43 & -12.37\% & 49 &  & 63 & 29.52\% \\
&\textbf{Total} & 1095 & -53.19\% & 2339 &  & 898 & -61.62\% \\ \hline
\multicolumn{2}{l}{\textbf{Synaptic Operations}} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff } & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff } \\ \hline
\textbf{Layer} & L0- & 2597 & -48.08\% & 5001 & 0.00\% & 12542 & 150.77\% \\
 & L1- & 10725 & -93.62\% & 168207 & 0.00\% & 8331 & -95.05\% \\
 & L2- & 43 & -12.37\% & 49 & 0.00\% & 63 & 29.52\% \\
&\textbf{Total} & 13365 & -92.29\% & 173257 & 0.00\% & 20936 & -87.92\%
\end{tabular}
\end{table}


==> tab/tab_comparison2_L2_apx.tex <==

% Energy-computations TABLE
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table}[]
\caption{Comparative synaptic operations and memory accesses per keyword averaged over the decoded whole dataset. Synaptic operations and memory access applied to L2, classification layer of LIF neurons for all architectures.  }
\label{tab:net_allComp_L2}
\begin{tabular}{llllllll}
 &  & \multicolumn{2}{l}{\textbf{TDE}} & \multicolumn{2}{l}{\textbf{LIFrec}} & \multicolumn{2}{l}{\textbf{LIF}} \\ \hline
\multicolumn{2}{l}{\textbf{Accuracy}} & \multicolumn{2}{c}{89.08 (1.25)} & \multicolumn{2}{c}{91.11 (1.07)} & \multicolumn{2}{c}{71.46 (0.44)} \\ \hline
\multicolumn{2}{l}{\textbf{\# cells (L2)}} & \multicolumn{2}{c}{11} & \multicolumn{2}{c}{11} & \multicolumn{2}{c}{11} \\ \hline
\multicolumn{2}{l}{\textbf{Spikes}} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} \\ \hline
\textbf{Layer} & L0 & \multicolumn{1}{l}{77} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{77} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{77} & \multicolumn{1}{l}{} \\
\textbf{} & L1 & 1124 & -66.61 & 3366 & 0.00 & 1291 & -61.66 \\
\textbf{} & L2 & 43 & -93.12 & 623 & 0.00 & 66 & -89.37 \\
\multicolumn{2}{l}{\textbf{Total}} & 1244 & -69.41 & 4066 & 0.00 & 1434 & -64.74 \\ \hline
\multicolumn{2}{l}{\textbf{Spike transmissions}} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Diff \%} \\ \hline
\textbf{From-layer-out} & L0 & 4771 & -79.33 & 7233 & -68.67 & 23083 & 0.00 \\
 & L1 & 12363 & -96.50 & 353425 & 0.00 & 14196 & -95.98 \\
 & L2 & 43 & -93.12 & 623 & 0.00 & 66 & -89.37 \\
\multicolumn{2}{l}{\textbf{Total}} & 17176 & -95.25 & 361281 & 0.00 & 37345 & -89.66 \\ \hline
\multicolumn{2}{l}{\textbf{SynOps}} & \# & Diff\% & \# & Diff\% & \# & Diff\% \\ \hline
\textbf{Total} & acc & 12406 & -67.05 & 37649 & 0.00 & 14262 & -62.12 \\
 & mac & 2200 & 0.00 & 2200 & 0.00 & 2200 & 0.00 \\
 & all & 14606 & -63.35 & 39849 & 0.00 & 16462 & -58.69 \\ \hline
\textbf{MemAcc} &  & \# & Diff\% & \# & Diff\% & \# & Diff\% \\ \hline
\textbf{Total} & Read & 29125 & -62.87 & 78451 & 0.00 & 32792 & -58.20 \\
\textbf{} & Write & 2243 & -20.56 & 2823 & 0.00 & 2266 & -19.73 \\
\textbf{} & all & 31368 & -61.40 & 81274 & 0.00 & 35058 & -56.86 \\ \hline
\end{tabular}
\end{table}





==> tab/tab_comparison2_v1.tex <==

% Energy-computations TABLE
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[ht]
\caption{Comparative table of synaptic operations and memory accesses for the tested architectures after training decoding the whole dataset.}
\label{tab:net_energy}
\begin{tabular}{lllllll}
\textbf{} & \multicolumn{2}{l}{\textbf{TDE}} & \multicolumn{2}{l}{\textbf{LIFrec}} & \multicolumn{2}{l}{\textbf{LIF}} \\ \hline
\textbf{Accuracy} & \multicolumn{2}{c}{87.86 (1.12)} & \multicolumn{2}{c}{90.04 (0.80)} & \multicolumn{2}{c}{71.59 (2.72)} \\ \hline
\textbf{\# cells (L1)} & \multicolumn{2}{c}{540} & \multicolumn{2}{c}{65} & \multicolumn{2}{c}{163} \\ \hline
\textbf{SynOps}                                        & \#              & Diff\%         & \#                & Diff\%       & \#              & Diff\%         \\ \hline
gain                                          &                 &                &                   &              &                 &                \\
acc                                           & 6031243         &                & 0                 &              & 0               &                \\
macc                                          & 594000          &                & 0                 &              & 0               &                \\
epsc                                          &                 &                &                   &              &                 &                \\
acc                                           & 6031243         &                & 691467205         &              & 58257341        &                \\
macc                                          & 594000          &                & 494000            &              & 179300          &                \\
mem                                           &                 &                &                   &              &                 &                \\
acc                                           & 594000          &                & 494000            &              & 179300          &                \\
macc                                          & 594000          &                & 494000            &              & 179300          &                \\
spks                                          & 49817427        &                & 781321800         &              & 38697318        &                \\
acc\_res                                      & 4528857         &                & 10280550          &              & 3517938         &                \\
Total                                         & 68784770        & -95.37         & 1484551555        & 0            & 101010497       & -93.20         \\ \hline
\textbf{MemAcc}                                        & \#              & Diff\%         & \#                & Diff\%       & \#              & Diff\%         \\ \hline
Read                                          &                 &                &                   &              &                 &                \\
RdSpkin                                       & 192999780       &                & 691467205         &              & 58257341        &                \\
RdPar                                         & 771999120       &                & 2074401615        &              & 174772023       &                \\
Rdtra                                         & 578999340       &                & 1382934410        &              & 116514682       &                \\
Write                                         &                 &                &                   &              &                 &                \\
WrSpk                                         & 540             &                & 65                &              & 163             &                \\
WrPot                                         & 578999340       &                & 1382934410        &              & 116514682       &                \\
Total                                         & 2122998120      & -61.62     & 5531737705        & 0            & 466058891       & -91.57     \\ \hline
 &  &  &  &  &  & 
\end{tabular}
\end{table}


